Uni-Sign: Toward Unified Sign Language Understanding at Scale

Sign language pre-training has gained increasing attention for its ability to enhance performance across various sign language understanding (SLU) tasks. However, existing methods often suffer from a gap between pre-training and fine-tuning, leading to suboptimal results. To address this, we propose Uni-Sign, a unified pre-training framework that eliminates the gap between pre-training and downstream SLU tasks through a large-scale generative pre-training strategy and a novel fine-tuning paradigm. First, we introduce CSL-News, a large-scale Chinese Sign Language (CSL) dataset containing 1,985 hours of video paired with textual annotations, which enables effective large-scale pre-training. Second, Uni-Sign unifies SLU tasks by treating downstream tasks as a single sign language translation (SLT) task during fine-tuning, ensuring seamless knowledge transfer between pre-training and fine-tuning. Furthermore, we incorporate a prior-guided fusion (PGF) module and a score-aware sampling strategy to efficiently fuse pose and RGB information, addressing keypoint inaccuracies and improving computational efficiency. Extensive experiments across multiple SLU benchmarks demonstrate that Uni-Sign achieves state-of-the-art performance across multiple downstream SLU tasks. Dataset and code are available at github.com/ZechengLi19/Uni-Sign.

==> Table/CSL_SLT.tex <==
\begin{table}[t]
    \centering
    \small
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{l|c|ccc|ccc}

    \toprule
    { \multirow{2}{*}{\tbf{Method}}} & \multirow{2}{*}{$\pmb{\mathcal{M}}$} & \multicolumn{3}{c|}{\tbf{Dev}}& \multicolumn{3}{c}{\tbf{Test}}\\
    & & BLEU1 & BLEU4 & ROUGE & BLEU1 & BLEU4 & ROUGE \\
    \midrule
        \rowcolor[gray]{.8} \multicolumn{8}{c}{Gloss-based}\\
    \midrule

    SLRT$^{\dagger}$~\citep{camgoz2020sign} &  \Rmodal & 37.47 &  11.88 &  37.96 &  37.38 & 11.79 &  36.74   \\
    
    ConSLT~\citep{ConSLT} &  \Rmodal & - & 14.80 & 41.46 & - &  14.53 & 40.98 \\
    
    SignBT~\citep{zhou2021improving} &  \Rmodal & 51.46 &  20.80 &  49.49 &  51.42 & 21.34 &  49.31  \\
    
    SLTUNET~\citep{zhang2023sltunet} &  \Rmodal & - & 23.99 & 53.58 & 54.98 &  25.01 & 54.08   \\
      
    MMTLB~\citep{chen2022simple}&  \Rmodal &  53.81 &  24.42 &  53.38 &  53.31 &    23.92 &  53.25  \\
     
    TS-SLT~\citep{chen2022two} &  \RPmodal &  \tbf{55.21} &  25.76 &  55.10 &  55.44 &   25.79 &  55.72  \\
    
    CV-SLT~\citep{zhao2024conditional} &  \Rmodal & - & \tbf{28.24} & \tbf{56.36} & \tbf{58.29}  & \tbf{28.94} & \tbf{57.06}  \\
    \midrule
        \rowcolor[gray]{.8} \multicolumn{8}{c}{Gloss-free}\\
    \midrule
    SLRT$^{\ddagger}$~\citep{camgoz2020sign} &  \Rmodal  &  21.03 &   4.04 &  20.51 &  20.00 &   3.03 &  19.67 \\
    
    GASLT~\citep{yin2023gloss} &  \Rmodal & - & - &  - &  19.90 &  4.07 &  20.35 \\
    
    NSLT$^{\dagger}$~\citep{cihan2018neural} &  \Rmodal &  34.22 & 7.96 &  34.28 &  34.16 &  7.56 &  34.54  \\
    
    MSLU~\citep{zhou2024scaling} &  \Pmodal& 33.28  & 10.27 & 33.13 & 33.97 & 11.42  & 33.80 \\
    
    GFSLT-VLP~\citep{zhou2023gloss} &  \Rmodal &  39.20 & 11.07 &  36.70 &  39.37 & 11.00 &  36.44  \\
    
    FLa-LLM~\citep{chen-etal-2024-fla-llm} &  \Rmodal &  - &  - &  - & 37.13 &  14.20 &  37.25  \\
    
    Sign2GPT~\citep{wong2024sign2gpt} &  \Rmodal &  - &  - &  - & {41.75} &  15.40 & {42.36} \\
    
    SignLLM~\citep{gong2024signllm} &  \Rmodal & \tbf{42.45} & \tbf{12.23} & \tbf{39.18} & {39.55} &  {15.75} & {39.91} \\
    
    {C$^2$RL}~\citep{chen2024c2rl}  & \Rmodal  & - & - & - & \tbf{49.32} &   \tbf{21.61} & \tbf{48.21} \\
    
    \midrule
    \modelname (Ours) &  \Pmodal& {53.24} & {25.27} & {54.34} & {53.86}  & {25.61} & {54.92} \\

    \modelname (Ours)& \RPmodal & \tbf{55.30}  & \tbf{26.25} & \tbf{56.03} &
    \tbf{55.08}  & \tbf{26.36} & \tbf{56.51} \\
     \bottomrule
    
    \end{tabular}
    \caption{\label{tab:exp csl-daily slt}SLT results on CSL-Daily dataset.
    \Rmodal and \Pmodal stand for RGB and pose as model inputs, respectively. 
    $\dagger$ denotes methods reproduced by \protect\citep{zhou2021improving}. 
    $\ddagger$ denotes methods reproduced by \protect\citep{zhou2023gloss}.}
    \vspace{-10pt}
\end{table}

\begin{wrapfigure}{r}{0.6\textwidth}
    \centering
    \small
    \setlength{\tabcolsep}{4pt}
    \resizebox{0.6\textwidth}{!}{
    \begin{tabular}{l|c|ccc|ccc}
    
    \toprule
    { \multirow{2}{*}{\tbf{Method}}} & \multirow{2}{*}{$\pmb{\mathcal{M}}$} & \multicolumn{3}{c|}{\tbf{Dev}} & \multicolumn{3}{c}{\tbf{Test}} \\
    & & BLEU1 & BLEU4 & ROUGE & BLEU1 & BLEU4 & ROUGE \\
    
    \midrule
        \rowcolor[gray]{.8} \multicolumn{8}{c}{Gloss-based} \\
    \midrule

    SLRT$^{\dagger}$~\citep{camgoz2020sign} &  \Rmodal & 37.47 & 11.88 & 37.96 & 37.38 & 11.79 & 36.74 \\
    ConSLT~\citep{ConSLT} &  \Rmodal & - & 14.80 & 41.46 & - & 14.53 & 40.98 \\
    SignBT~\citep{zhou2021improving} &  \Rmodal & 51.46 & 20.80 & 49.49 & 51.42 & 21.34 & 49.31 \\
    SLTUNET~\citep{zhang2023sltunet} &  \Rmodal & - & 23.99 & 53.58 & 54.98 & 25.01 & 54.08 \\
    MMTLB~\citep{chen2022simple} &  \Rmodal & 53.81 & 24.42 & 53.38 & 53.31 & 23.92 & 53.25 \\
    TS-SLT~\citep{chen2022two} &  \RPmodal & \tbf{55.21} & 25.76 & 55.10 & 55.44 & 25.79 & 55.72 \\
    CV-SLT~\citep{zhao2024conditional} &  \Rmodal & - & \tbf{28.24} & \tbf{56.36} & \tbf{58.29} & \tbf{28.94} & \tbf{57.06} \\
    
    \midrule
        \rowcolor[gray]{.8} \multicolumn{8}{c}{Gloss-free} \\
    \midrule
    SLRT$^{\ddagger}$~\citep{camgoz2020sign} &  \Rmodal & 21.03 & 4.04 & 20.51 & 20.00 & 3.03 & 19.67 \\
    GASLT~\citep{yin2023gloss} &  \Rmodal & - & - & - & 19.90 & 4.07 & 20.35 \\
    NSLT$^{\dagger}$~\citep{cihan2018neural} &  \Rmodal & 34.22 & 7.96 & 34.28 & 34.16 & 7.56 & 34.54 \\
    MSLU~\citep{zhou2024scaling} &  \Pmodal & 33.28 & 10.27 & 33.13 & 33.97 & 11.42 & 33.80 \\
    GFSLT-VLP~\citep{zhou2023gloss} &  \Rmodal & 39.20 & 11.07 & 36.70 & 39.37 & 11.00 & 36.44 \\
    FLa-LLM~\citep{chen-etal-2024-fla-llm} &  \Rmodal & - & - & - & 37.13 & 14.20 & 37.25 \\
    Sign2GPT~\citep{wong2024sign2gpt} &  \Rmodal & - & - & - & 41.75 & 15.40 & 42.36 \\
    SignLLM~\citep{gong2024signllm} &  \Rmodal & \tbf{42.45} & \tbf{12.23} & \tbf{39.18} & 39.55 & 15.75 & 39.91 \\
    {C$^2$RL}~\citep{chen2024c2rl} & \Rmodal & - & - & - & \tbf{49.32} & \tbf{21.61} & \tbf{48.21} \\
    
    \midrule
    \modelname (Ours) & \Pmodal & {53.24} & {25.27} & {54.34} & {53.86} & {25.61} & {54.92} \\
    \modelname (Ours) & \RPmodal & \tbf{55.30} & \tbf{26.25} & \tbf{56.03} & \tbf{55.08} & \tbf{26.36} & \tbf{56.51} \\
    
    \bottomrule
    \end{tabular}
    }
    \caption{\label{tab:exp csl-daily slt} SLT results on CSL-Daily dataset. \Rmodal and \Pmodal stand for RGB and pose as model inputs, respectively. $\dagger$ and $\ddagger$ denote methods reproduced by \protect\citep{zhou2021improving} and \protect\citep{zhou2023gloss}.}
    \vspace{-10pt}
\end{wrapfigure}


==> Table/ENXX_SLT.tex <==
\begin{table}[t]
    \centering
    \small
    \setlength{\tabcolsep}{4pt}

    \begin{tabular}{l|c|ccccc}
    
    \toprule
    {{\tbf{Method}}} & {$\pmb{\mathcal{M}}$} & BLEU1  & BLEU2 & BLEU4 & ROUGE & BLEURT \\
    \midrule
        \rowcolor[gray]{.8} \multicolumn{7}{c}{How2Sign}\\
    \midrule

    GloFE-VN~\citep{lin-etal-2023-GloFE} & \Pmodal& 14.9 & 7.3 & 2.2 & 12.6 & 31.7 \\
    
    MSLU~\citep{zhou2024scaling} & \Pmodal& 20.1 & 7.7 & 2.4 & 17.2 & - \\
    
    SLT-IV~\citep{tarres2023sign-instructional} & \Rmodal & 34.0 & 19.3  & 8.0 & -  & - \\
    
    {C$^2$RL}~\citep{chen2024c2rl} & \Rmodal &  29.1 & 18.6 & 12.9 & 27.0 & - \\
    
    FLa-LLM~\citep{chen-etal-2024-fla-llm} & \Rmodal &  29.8  & 19.0 &  9.7 &  27.8  \\
    
    YouTube-ASL~\citep{uthus2024ytasl} & \Pmodal&  37.8 &  24.1 &    12.4  &  - & 46.6 \\
    
    SignMusketeers~\citep{gueuwou2024signmusketeers} & \Rmodal & 41.5 & 27.2 & 14.3 & - & - \\
    
    SSVP-SLT~\citep{rust-etal-2024-ssvp} & \Rmodal &  \tbf{43.2} & \tbf{28.8}  &  15.5 & \tbf{38.4} & 49.6 \\
    
    SSLT$^\dagger$~\citep{zhang2024scalingslt} & \Pmodal&  - & - &  \tbf{21.1} & - & \tbf{55.7} \\
    
    \midrule
    \modelname (Ours) &  \Pmodal &  \tbf{40.4} & 26.8 & 14.5 & 34.3 & 48.6 \\
    \modelname (Ours) &  \RPmodal & 40.2 & \tbf{27.1} & \tbf{14.9} & \tbf{36.0} & \tbf{49.4}   \\
    
    \midrule
        \rowcolor[gray]{.8} \multicolumn{7}{c}{OpenASL}\\
    \midrule
    Conv-GRU$^{\dagger}$~\citep{cihan2018neural} & \Rmodal & 16.11 & 8.85 & 4.58 & 16.10 & 25.65 \\

    I3D-transformer~\citep{shi-etal-2022openasl} & \Rmodal  & 18.31 & 10.15 & 5.66 & 18.64 & 28.82 \\
    
    OpenASL~\citep{shi-etal-2022openasl} & \Rmodal & 20.92 & 12.08 & 8.59 & 21.02 & 31.09 \\
    
    GloFE-VN~\citep{lin-etal-2023-GloFE} & \Pmodal & 21.56 & 12.74 & 7.06 & 21.75 & \tbf{36.35} \\
    
    {C$^2$RL}~\citep{chen2024c2rl} & \Rmodal & \tbf{31.46} & \tbf{21.85} & \tbf{13.21} & \tbf{31.36} & -\\
    
    \midrule
    \modelname (Ours) & \Pmodal & 
    49.10 & 35.91 & 22.67 & 42.77 & 60.08 \\

    \modelname (Ours)  &  \RPmodal & 
    \tbf{49.35} & \tbf{36.32} & \tbf{23.14} & \tbf{43.22} & \tbf{60.40} \\
    \bottomrule
    
  \end{tabular}
    \caption{\label{tab:exp how2sign & openasl slt}Gloss-free SLT results on How2Sign and OpenASL dataset.
    $\dagger$ denotes training with an additional large-scale dataset.}
    \vspace{-10pt}
\end{table}

\begin{wrapfigure}{r}{0.6\textwidth} 
    \vspace{-1em} 
    \centering
    \resizebox{0.6\textwidth}{!}{ 
        \begin{tabular}{l|c|ccccc}
        
        \toprule
        {{\tbf{Method}}} & {$\pmb{\mathcal{M}}$} & BLEU1  & BLEU2 & BLEU4 & ROUGE & BLEURT \\
        \midrule
            \rowcolor[gray]{.8} \multicolumn{7}{c}{How2Sign}\\
        \midrule

        GloFE-VN~\citep{lin-etal-2023-GloFE} & \Pmodal& 14.9 & 7.3 & 2.2 & 12.6 & 31.7 \\
        
        MSLU~\citep{zhou2024scaling} & \Pmodal& 20.1 & 7.7 & 2.4 & 17.2 & - \\
        
        SLT-IV~\citep{tarres2023sign-instructional} & \Rmodal & 34.0 & 19.3  & 8.0 & -  & - \\
        
        {C$^2$RL}~\citep{chen2024c2rl} & \Rmodal &  29.1 & 18.6 & 12.9 & 27.0 & - \\
        
        FLa-LLM~\citep{chen-etal-2024-fla-llm} & \Rmodal &  29.8  & 19.0 &  9.7 &  27.8  \\
        
        YouTube-ASL~\citep{uthus2024ytasl} & \Pmodal&  37.8 &  24.1 &    12.4  &  - & 46.6 \\
        
        SignMusketeers~\citep{gueuwou2024signmusketeers} & \Rmodal & 41.5 & 27.2 & 14.3 & - & - \\
        
        SSVP-SLT~\citep{rust-etal-2024-ssvp} & \Rmodal &  \tbf{43.2} & \tbf{28.8}  &  15.5 & \tbf{38.4} & 49.6 \\
        
        SSLT$^\dagger$~\citep{zhang2024scalingslt} & \Pmodal&  - & - &  \tbf{21.1} & - & \tbf{55.7} \\
        
        \midrule
        \modelname (Ours) &  \Pmodal &  \tbf{40.4} & 26.8 & 14.5 & 34.3 & 48.6 \\
        \modelname (Ours) &  \RPmodal & 40.2 & \tbf{27.1} & \tbf{14.9} & \tbf{36.0} & \tbf{49.4}   \\
        
        \midrule
            \rowcolor[gray]{.8} \multicolumn{7}{c}{OpenASL}\\
        \midrule
        Conv-GRU$^{\dagger}$~\citep{cihan2018neural} & \Rmodal & 16.11 & 8.85 & 4.58 & 16.10 & 25.65 \\

        I3D-transformer~\citep{shi-etal-2022openasl} & \Rmodal  & 18.31 & 10.15 & 5.66 & 18.64 & 28.82 \\
        
        OpenASL~\citep{shi-etal-2022openasl} & \Rmodal & 20.92 & 12.08 & 8.59 & 21.02 & 31.09 \\
        
        GloFE-VN~\citep{lin-etal-2023-GloFE} & \Pmodal & 21.56 & 12.74 & 7.06 & 21.75 & \tbf{36.35} \\
        
        {C$^2$RL}~\citep{chen2024c2rl} & \Rmodal & \tbf{31.46} & \tbf{21.85} & \tbf{13.21} & \tbf{31.36} & -\\
        
        \midrule
        \modelname (Ours) & \Pmodal & 
        49.10 & 35.91 & 22.67 & 42.77 & 60.08 \\

        \modelname (Ours)  &  \RPmodal & 
        \tbf{49.35} & \tbf{36.32} & \tbf{23.14} & \tbf{43.22} & \tbf{60.40} \\
        \bottomrule
      \end{tabular}
    }
    \caption{\label{tab:exp how2sign & openasl slt}Gloss-free SLT results on How2Sign and OpenASL dataset.
    $\dagger$ denotes training with an additional large-scale dataset.}
    \vspace{-10pt} 
\end{wrapfigure}

